Excited-state hydroxyl maser catalogue from the methanol multibeam survey -- I. Positions and Variability

We present the results of the first complete unbaised survey of the Galactic Plane for 6035-MHz excited-state hydroxyl masers undertaken as part of the Methanol Multibeam Survey. These observations cover the Galactic longitude ranges $186^{\circ}< l < 60^{\circ}$ including the Galactic Centre. We report the detection of 127 excited-state hydroxyl masers within the survey region, 47 being new sources. The positions of new detections were determined from interferometric observations with the Australia Telescope Compact Array. We discuss the association of 6035-MHz masers in our survey with the 6668-MHz masers from the MMB Survey, finding 37 likely methanol-excited-state hydroxyl masers maser pairs with physical separations of <=0.03pc and 55 pairings separated by <=0.1pc. Using these we calculate for the first time an excited-state hydroxyl maser life time of between 3.3x10^3 and 8.3x10^3 years. We also discuss the variability of the 6035-MHz masers and detection rates of counterpart 6030-MHz excited-state hydroxyl masers (28% of our sample having detection at both frequencies).

==> exOH_spectra_2016_short.tex <==
\newpage
\onecolumn
\begin{figure}
\centering
	\subfloat[\textit{MMBOH-G000.666-00.029 \& MMBOH-G000.666-00.035}]{\includegraphics[width=0.33\textwidth]{redblue_MX_plots/MMBOH-G000p666-00p035.eps}}
	\subfloat[\textit{MMBOH-G004.682+00.278}]{\includegraphics[width=0.33\textwidth]{redblue_MX_plots/MMBOH-G004p682+00p278.eps}}
	\subfloat[\textit{MMBOH-G005.885-00.392}]{\includegraphics[width=0.33\textwidth]{redblue_MX_plots/MMBOH-G005p885-00p392.eps}}
\qquad
	\subfloat[\textit{MMBOH-G006.882+00.094}]{\includegraphics[width=0.33\textwidth]{redblue_MX_plots/MMBOH-G006p882+00p094.eps}}
	\subfloat[\textit{MMBOH-G008.352+00.478}]{\includegraphics[width=0.33\textwidth]{redblue_MX_plots/MMBOH-G008p352+00p478.eps}}
	\subfloat[\textit{MMBOH-G008.669-00.356}]{\includegraphics[width=0.33\textwidth]{redblue_MX_plots/MMBOH-G008p669-00p356.eps}}
\qquad
	\subfloat[\textit{MMBOH-G009.620+00.194 \& MMBOH-G009.622+00.196}]{\includegraphics[width=0.33\textwidth]{redblue_MX_plots/MMBOH-G009p620+00p194.eps}}
	\subfloat[\textit{MMBOH-G010.322-00.258}]{\includegraphics[width=0.33\textwidth]{redblue_MX_plots/MMBOH-G010p322-00p258.eps}}
	\subfloat[\textit{MMBOH-G010.623-00.384}]{\includegraphics[width=0.33\textwidth]{redblue_MX_plots/MMBOH-G010p623-00p384.eps}}
\qquad
	\subfloat[\textit{MMBOH-G010.960+00.022}]{\includegraphics[width=0.33\textwidth]{redblue_MX_plots/MMBOH-G010p960+00p022.eps}}
	\subfloat[\textit{MMBOH-G011.034+00.062}]{\includegraphics[width=0.33\textwidth]{redblue_MX_plots/MMBOH-G011p034+00p062.eps}} 
	\subfloat[\textit{MMBOH-G011.904-00.141}]{\includegraphics[width=0.33\textwidth]{redblue_MX_plots/MMBOH-G011p904-00p141.eps}}
	\caption{MMB ex-OH maser spectra from the Parkes `MX' observations. Red (solid) and blue (dashed) lines are right and left hand circular polarisations respectively. Spectra for two sources are presented (\textit{49.046$-$0.290} and \textit{326.447$-$0.749}) in black (dash-dot) lines, these are Stokes I spectra from ATCA as these sources are not present in the nearest Parkes MX. The full version of this figure is available in the online version of this paper.}
	\label{abcd}
\end{figure}

